Generalized Section-Section Interaction Potentials in the Geometrically Exact Beam Theory: Modeling of Intermolecular Forces, Asymptotic Limit as Strain-Energy Function, and Formulation of Rotational Constraints

The present contribution proposes a universal framework to formulate generalized section-section interaction potentials (SSIP) within the geometrically exact beam theory. By exploiting the fundamental kinematic assumption of undeformable cross-sections, an objective (i.e., frame-invariant) description of SSIPs via a minimal set of six (translational and rotational) relative coordinates, either in spatial or in material form, is proposed. Based on work-pairing, work-conjugated section-section interaction forces and moments, either in spatial or in material form, are identified that can be consistently derived from a variational principle. Interestingly, it is shown that hyperelastic stored-energy functions relating the deformation measures and stress-resultants of the well-known geometrically exact Simo-Reissner beam theory can also be identified as SSIPs when considering the asymptotic limit of small relative distances and rotations between the interacting cross-sections. Moreover, the proposed variational problem formulation is demonstrated to be of a very general nature, thus allowing for the formulation of translational and rotational constraints between arbitrarily oriented cross-sections based on either a penalty or a Lagrange multiplier potential. Possible applications include fiber-based structures and materials in technical and biological systems, where the proposed approach allows to model short- or long-ranged inter-molecular (e.g., electrostatic, van der Waals or repulsive steric) interactions between fibers in geometrically complex arrangements and to formulate translational and rotational coupling constraints between different fibers (e.g., cross-linked polymer chains) or between fibers and a matrix phase (e.g., fiber-reinforced composites).

==> 01_sections/20_theory.tex <==
% !TEX root = ../Cosserat_interaction_potential.tex

\section{Generalized section-section interaction potentials}
%
\subsection{Kinematics}
\label{sec:kinematics}

The overall interaction potential between two beams shall be given by the integral of the molecule-to-molecule interaction potential $\Phi(x)$ over the volumes $V_1$ and $V_2$ of the interacting beams:
%
\begin{align}
\label{potential_1}
  \Pi = \int_{l_1} \int_{l_2} \underbrace{\int_{A_1} \int_{A_2} \rho_1(\vs_1) \rho_2(\vs_2) \Phi(x) \dd A_2 \dd A_1}_{\pi} \dd l_2 \dd l_1.
\end{align}
%
Here, $A_i$, $l_i$ and $\rho_i$ represent the cross-section area, the length, and the molecule density of beam $i$. From a physical point of view, the integral of $\Phi(x)$ over the two beam cross-sections (weighted by the molecule densities $\rho_1(\vs_1)$ and $\rho_2(\vs_2)$) represents the net interaction between two cross-sections, and shall be denoted as section interaction potential $\pi$ in the following. Moreover, $x$ is the distance between the two interacting volume elements $dA_1 \cdot dl_1$ and $dA_2 \cdot dl_2$, and is defined as:
%
\begin{align}
\label{x21}
  x = \norm{\vx_{21}} \quad \text{with} \quad \vx_{21} = \vx_2 - \vx_1
\end{align}
%
The basic kinematic assumption of the geometrically exact beam theory allows to express the position $\vx_i$ of an arbitrary point within the cross-section of beam $i$ as
\begin{align}
\label{xi}
  \vx_i = \vr_i(s_i^1) + \underbrace{s_i^2 \vg_i^2 + s_i^3 \vg_i^3}_{=: \vs_i}, \quad i=1,2,
\end{align}
%
where $\vr_i(s_i^1)$ represents the cross-section centroid position, $(g_i^1, g_i^2, g_i^3)$ are the base vectors of a right-handed, orthonormal basis $\vLambda_i$ attached to the cross-section of beam $i$ with $g_i^2$ and $g_i^3)$ representing the principle axes of intertia of area. Alternatively, $\vLambda_i \in SO(3)$ can be interpreted as a rotation tensor from the fixed, Euclidean basis $(e^1,e^2,e^3)$ to the moving (body-fixed) triad $(g_i^1, g_i^2, g_i^3)$. Moreover, $s_i^1$ is a convective (arc-length) coordinate in beam length direction, i.e. $dl_i=ds_i^1$, $s_i^2$ and $s_i^3$ are convective coordinates in $g_i^2$ and $g_i^3$-direction spanning the cross-section, i.e. $dA_i=s_i^2s_i^3$. Eventually, $\vs_i$ is the distance between an arbitrary point within the cross-section of beam $i$ and its centroid. In a next step, let's define the relative distance $\vr_{21}$ between the two cross-section centroids as well as the relative rotation $\vLambda_{12} = \exp{\!(\vS(\vpsi_{21}))}$ between the two cross-section triads:
%
\begin{subequations}
\label{d_and_psi}
\begin{align}
  \vr_{21} := \vr_2 - \vr_1 \quad & \Leftrightarrow \quad \vr_2 = \vr_1 + \vr_{21}\\
  \vLambda_{21} := \vLambda_2 \vLambda_1^\text{T} \quad & \Leftrightarrow \quad \vLambda_2 = \vLambda_{21} \vLambda_1 \quad \text{or} \quad \vg_2^i = \vLambda_{21} \, \vg_1^i \quad \text{for} \quad  i=1,2,3
\end{align}
\end{subequations}
%
As exemplary rotation parametrization, the rotation (pseudo-)vector $\vpsi_{21}$ has been chosen. Moreover, an exemplary coordinate representation w.r.t. to the basis $\vLambda_1$ shall be given for these kinematic quantities:
%
\begin{align}
\label{d_and_psi_2}
  \vr_{21} =: r_{21}^i\vg_1^i, \quad  \vpsi_{21} =: \psi_{21}^i\vg_1, \quad  \vLambda_{21} =: \Lambda_{21}^{ij} \vg_1^{i} \otimes \vg_1^{jT}
\end{align}
%
Here and in the following, double indices imply summation over the index range. Making use of~\eqref{x21},~\eqref{xi} and~\eqref{d_and_psi}, the distance vector $\vx_{21}$ between two interacting volumes can be rewritten to
%
\begin{align}
\begin{split}
\label{x21_final}
  \vx_{21} &= \vr_2 - \vr_1 + \left( s_2^2 \vg_2^2 + s_2^3 \vg_2^3 \right) - \left( s_1^2 \vg_1^2 + s_1^3 \vg_1^3 \right)\\
  &= \vr_{21} + \vLambda_{21} \left( s_2^2 \vg_1^2 + s_2^3 \vg_1^3 \right) - \left( s_1^2 \vg_1^2 + s_1^3 \vg_1^3 \right).
\end{split}
\end{align}
%
When considering~\eqref{x21_final} together with~\eqref{d_and_psi_2} the following statement can be made: The distance vector $\vx_{21}$ between two given cross-section points $(s_1^2,s_1^3)$ and $(s_2^2,s_2^3)$, e.g. expressed in the basis $\vLambda_1$ according to $\vx_{21}=:x_{21}^ig_1^i$ with known base vectors $g_1^i$, is uniquely defined by the relative position and rotation vectors $\vr_{21}$ and $\vpsi_{21}$ (used for parameterization of $\vLambda_{21}$). Consequently, as expected, after integrating over the four cross-section coordinates $s_i^2$ and $s_i^3$ in~\eqref{potential_1}, the resulting section interaction potential is a pure function of the six relative degrees of freedom between the interacting cross-sections, i.e. $\pi=\tilde{\pi}(\vr_{21},\vpsi_{21})$. In other words, $\vr_{21}$ and $\vpsi_{21}$ can be interpreted as generalized (spatial) deformation measures uniquely describing the considered interaction potential. By defining $\vLambda_1$ and  $\vLambda_1^T$ as push-forward and pull-back operator, also a material representation of these deformation measures can be stated:
%
\begin{align}
\label{D_and_Psi}
  \vr_{21}:=\vLambda_1\vR_{21}, \,\, \vpsi_{21}=\vLambda_1\vPsi_{21}  \quad \Leftrightarrow \quad \vR_{21}:=\vLambda_1^T\vr_{21}, \,\,\vPsi_{21}=\vLambda_1^T\vpsi_{21}.
\end{align}
%
Making use of~\eqref{d_and_psi}, the rotation tensor $\vLambda_{\mathbbm{2}\mathbbm{1}} := \exp{\!(\vS(\vPsi_{21}))}$ associated with $\vPsi_{21}$ can be written as
\begin{align}
\label{Lambda_Psi}
  \vLambda_{\mathbbm{2}\mathbbm{1}} := \exp{\!(\vS(\vLambda_1^T \vpsi_{21}))}  = \vLambda_1^T  \exp{\!(\vS(\vpsi_{21}))} \vLambda_1 = \vLambda_1^T \vLambda_{21} \vLambda_1 = \vLambda_1^T \vLambda_2 \quad \Leftrightarrow \quad \vLambda_2 =  \vLambda_1\vLambda_{\mathbbm{2}\mathbbm{1}},
\end{align}
%
where~\eqref{A_Lambda1} has been exploited from the second to the third expression. Thus, the spatial quantity $\vpsi_{21}$ defines the relative rotation via left-multiplication of $\vLambda_1$, while the material quantity $\vPsi_{21}$ defines it via right-multiplication of $\vLambda_1$. Considering the coordinate representations~\eqref{d_and_psi_2}, we get
%
\begin{align}
\label{D_and_Psi_2}
  \vR_{21} = r_{21}^i\ve_1^i, \quad  \vPsi_{21} = \psi_{21}^i\ve_1, \quad  \vLambda_{\mathbbm{2}\mathbbm{1}} = \Lambda_{21}^{ij} \ve^{i} \otimes \ve^{jT}
\end{align}
Thus, the coordinates of the material deformation measures when expressed in the inertial frame $\ve^{i}$ are identical to the coordinates of the spatial deformation measures when expressed in the moving frame $g_1^{i}$. With these results at hand, also the distance vector $\vx_{21}$ 
can be back-rotated according to:
%
\begin{align}
\begin{split}
\label{X21_final}
  \vX_{21}:= \vLambda_1^T \vx_{21} &= \vLambda_1^T \vr_{21} + \vLambda_1^T \vLambda_{21} \left( s_2^2 \vg_1^2 + s_2^3 \vg_1^3 \right) - \vLambda_1^T \left( s_1^2 \vg_1^2 + s_1^3 \vg_1^3 \right)\\
  &=\vLambda_1^T \vr_{21} + \vLambda_1^T \vLambda_{21}  \vLambda_1 \vLambda_1^T \left( s_2^2 \vg_1^2 + s_2^3 \vg_1^3 \right) - \vLambda_1^T \left( s_1^2 \vg_1^2 + s_1^3 \vg_1^3 \right)\\
  &=\vR_{21} +  \vLambda_{\mathbbm{2}\mathbbm{1}} \left( s_2^2 \ve^2 + s_2^3 \ve^3 \right) -  \left( s_1^2 \ve^2 + s_1^3 \ve^3 \right)
\end{split}
\end{align}
%
Together with~\eqref{D_and_Psi_2} it becomes clear that the coordinates of the distance vector $\vX_{21}$ in the basis $e_1^i$, i.e. $\vX_{21}=\vLambda_1^T \vx_{21}=:x_{21}^ie_1^i$, are a pure function of $\vR_{21}$ and $\vPsi_{21}$ (or more precisely, of their six coordinates in the basis $\ve^i$). Because the back-rotation $\vX_{21}:= \vLambda_1^T \vx_{21}$ preserves the $L_2-$norm, i.e. $\norm{\vX_{21}}=\norm{\vLambda_1^T \vx_{21}}=\norm{\vx_{21}}=x$, the molecule-to-molecule interaction potential $\Phi$ can equivalently be written as $\Phi(x)=\Phi(\norm{\vx_{21}})=\Phi(\norm{\vX_{21}})$. The section-to-section interaction potential $\pi$, however, will in general be a function of the vectors $(\vr_{21},\vpsi_{21})$ or  $(\vR_{21},\vPsi_{21})$, but not only of their norms. Thus, the corresponding functional expressions $\tilde{\pi}$ and $\bar{\pi}$ in spatial and material configuration will be different in general:
\begin{align}
\label{barbar_pi}
\tilde{\pi}(\vr_{21},\vpsi_{21})=\tilde{\pi}(\vLambda_1\vR_{21},\vLambda_1\vPsi_{21})={\bar{\pi}}(\vR_{21},\vPsi_{21}).
\end{align}

In preparation to the following variational formulation of the considered beam-to-beam interaction problem, the variation of the introduced kinematic quantities will be required. Based on a parameterization with the rotation vector~$\vpsi$, the variation of the rotation tensor reads:
\begin{align}
\label{largerotations_deltalambdaspatial}
  \delta \vLambda =: \frac{d}{d \epsilon} \Big|_{\epsilon=0}  \vLambda ( \vpsi + \epsilon \delta \vpsi)  = \frac{\partial \vLambda (\vpsi)}{\partial \vpsi} \delta \vpsi.
\end{align}
Alternatively, the variation of the rotation tensor may be expressed as
\begin{align}
\label{multi_var}
\delta \vLambda =: 
  \frac{d}{d \epsilon} \Big|_{\epsilon=0} \left[ \vLambda (\epsilon \delta \vtheta) \vLambda \right]
  = \vS(\delta \vtheta) \vLambda(\vpsi),
\end{align}
where $\delta \vtheta$ is typically denoted as multiplicative rotation vector variation or spin vector. Moreover, $\vS$ represents a skew symmetric matrix, i.e. $\vS=-\vS^T$, with $\vS(\va)\vb \!=\!\va\!\times\!\vb \,\, \text{for} \,\, \va,\vb  \!\in\! \Re^3$. With~\eqref{multi_var}, the variation of the base vectors $\vg^i$ can be formulated as
\begin{align}
\label{multi_var_base}
\delta \vg^i = \vS(\delta \vtheta) \vg^i = \delta \vtheta \times \vg^i.
\end{align}
The additive and multiplicative variations are related by the well-known transformation matrix $\vT( \vpsi)$:
\begin{align}
\label{Tmatrix}
\delta \vpsi = \vT( \vpsi) \delta \vtheta.
\end{align}
By expressing the variation of an arbitrary function $\vf(\vpsi)$ via the multiplicative rotation vector variation $\delta \vtheta$ and making use of~\eqref{Tmatrix}, we define the \textit{multiplicative derivative} $\partial_m \vf / \partial_m \vtheta$ of this function as:
\begin{align}
\label{multiplicative_derivative}
\delta \vf = \frac{\partial \vf}{\partial \vpsi} \delta \vpsi = \frac{\partial \vf}{\partial \vpsi} \vT( \vpsi) \delta \vtheta=:\frac{\partial_m \vf}{\partial_m \vtheta} \delta \vtheta 
\quad \Leftrightarrow \quad \frac{\partial_m \vf}{\partial_m \vtheta}:=\frac{\partial \vf}{\partial \vpsi} \vT( \vpsi),
\end{align}
where $\partial \vf / \partial \vpsi$ is the standard partial (or additive) derivative of $\vf(\vpsi)$. In order to derive the weak form of the mechanical balance equations for geometrically exact beam model on the basis of a variational principle, the variations of the material deformation measures $\vR_{21}$ and $\vPsi_{21}$ have to be expressed via the spatial variations of the beam cross-section centroid positions $\delta \vr_1$ and $\delta \vr_2$ and the (spatial) spin vectors $\delta \vtheta_1$ and $\delta \vtheta_2$ associated with the cross-section triads of beam $1$ and $2$. A straightforward calculation leads to the following expression for the variation of the material deformation measures $\vR_{21}$ and $\vPsi_{21}$:
\begin{subequations}
\label{delta_material}
\begin{align}
  \delta \vR_{21} &= \vLambda_1^T \left( \delta \vr_2 - \delta \vr_1 + \left( \vr_2 - \vr_1 \right) \times \delta \vtheta_1 \right)\\
  \delta \vPsi_{21} &= \vT(\vPsi_{21}) \delta \vTheta_{21} = \vT(\vPsi_{21}) \vLambda_1^T \left( \delta \vtheta_2 - \delta \vtheta_1 \right),
\end{align}
\end{subequations}
where the multiplicative variation $\delta \vTheta_{21}:=\vLambda_1^T \left( \delta \vtheta_2 - \delta \vtheta_1 \right)$ has been defined in accordance to~\eqref{multi_var}, i.e.
\begin{align}
\label{multi_var_21}
\delta \vLambda_{\mathbbm{2}\mathbbm{1}} =: \vS(\delta \vTheta_{21}) \vLambda_{\mathbbm{2}\mathbbm{1}}.
\end{align}
The objective variation of an arbitrary spatial quantity $\va$ shall be defined as the difference between the total variation and the variation due to variation of the base vectors if expressed in the moving frame $\vLambda_1$, i.e. $\delta_o \va:=\delta \va - \delta \vtheta_1 \times \va=\delta \va - \vS(\delta \vtheta_1) \va$.  Based on this definition it can be shown that the objective variations of the deformation measures $\vr_{21}$ and $\vpsi_{21}$ are given by:
\begin{subequations}
\label{delta_o}
\begin{align}
  \delta_o \vr_{21} &:= \delta \vr_{21} - \delta \vtheta_1 \times \vr_{21} = \underbrace{\left( \delta \vr_2 - \delta \vr_1 + \left( \vr_2 - \vr_1 \right) \times \delta \vtheta_1 \right)}_{\vLambda_1 \delta \vR_{21}} \label{delta_o_1} \\
  \delta_o \vpsi_{21} &:= \delta \vpsi_{21} - \delta \vtheta_1 \times \vpsi_{21} =  \underbrace{\vLambda_1 \vT(\vPsi_{21}) \vLambda_1^T \left( \delta \vtheta_2 - \delta \vtheta_1 \right)}_{\vLambda_1 \delta \vPsi_{21}}
  =  \vT(\vpsi_{21}) \left( \delta \vtheta_2 - \delta \vtheta_1 \right).\label{delta_o_2}
\end{align}
\end{subequations}
Thus, as expected, the objective variations of the spatial deformation measures are the push-forward of the variations of the material deformation measures. In the last reformulation step, used has been made of utility equation~\eqref{A_T1}. Using the last expression in the second line,~\eqref{delta_o_2} can be reformulated to
\begin{align}
  \delta_o \vpsi_{21} =  \vT(\vpsi_{21}) \left( \delta \vtheta_2 - \delta \vtheta_1 \right) =: \vT(\vpsi_{21}) \delta_o \vtheta_{21},
\end{align}
where the objective multiplicative variation $\delta_o \vtheta_{21}:=\delta \vtheta_2 - \delta \vtheta_1$ has been defined in accordance to~\eqref{multi_var}:
\begin{align}
\label{multi_var_21}
\delta_o \vLambda_{21} =: \vS(\delta_o \vtheta_{21}) \vLambda_{21}.
\end{align}
Here, similar to the objective variation of a spatial vector, the objective variation of the spatial relative rotation tensor $\vLambda_{21}$ has been defined as the difference between the total variation and the variation due to variation of the base vectors if expressed in the moving frame $\vLambda_1$ (see~\eqref{d_and_psi_2}):
\begin{align}
\delta_o \vLambda_{21}:=\delta \vLambda_{21} - (\Lambda_{21}^{ij} \delta \vg_1^{i} \otimes \vg_1^{jT} + \Lambda_{21}^{ij}  \vg_1^{i} \otimes \delta \vg_1^{jT})=\delta \vLambda_{21} - (\vS(\delta \vtheta_1) \vLambda_{21}  + \vLambda_{21} \vS(\delta \vtheta_1)^T).
\end{align}

\begin{center}
\begin{minipage}{0.9\textwidth}
{
\noindent \textbf{Remark:} With the coordinate representations~\eqref{d_and_psi_2} and~\eqref{D_and_Psi_2}, the objective variation of the spatial relative rotation tensor $\vLambda_{21}$ can alternatively be expressed as push-forward of the variation of the material relative rotation tensor $\vLambda_{\mathbbm{2}\mathbbm{1}}$, i.e. $\delta_o \vLambda_{21}= \delta \Lambda_{21}^{ij} \vg_1^{i} \otimes \vg_1^{jT} = \vLambda_{1} \delta \vLambda_{\mathbbm{2}\mathbbm{1}} \vLambda_{1}^T$.
}
\end{minipage}
\end{center}


\subsection{Stress resultants and weak form of the balance eqations}

From the molecule-to-molecule interaction potential $\Phi(x)=\Phi(\norm{x_{21}})$ the molecule-to-molecule interaction forces on molecule $1$ and molecule $2$ are defined as
\begin{align}
  \vf_{m1} = -  \pdiff{\Phi}{{\vx_{21}}} \quad \text{and} \quad \vf_{m2} = \pdiff{\Phi}{{\vx_{21}}}=-\vf_m1.
\end{align}
In a similar fashion, the differential force resultants between two differential volume elements $dA_1dl_1$ and $dA_2 dl_2$ at positions $\vx_1$ and $\vx_2$ within the cross-sections $A_1$ and $A_2$ is given by
\begin{subequations}
\begin{align}
  \dd \vf_{dA_1dl_1}(\vx_1) &= - \rho_1(\vs_1) \rho_2(\vs_2) \pdiff{\Phi}{{\vx_{21}}} \dd A_2 \dd A_1 dl_2 dl_1\\
  \dd \vf_{dA_2dl_2}(\vx_2) &= \rho_1(\vs_1) \rho_2(\vs_2) \pdiff{\Phi}{{\vx_{21}}} \dd A_2 \dd A_1 dl_2 dl_1 = -\dd \vf_{dA_1dl_1}(\vx_1)
\end{align}
\end{subequations}
Integration over the two cross-sections yields the resulting differential force resultant between two cross-section slices with areas $A_1$ and $A_2$ and thicknesses $dl_1$ and $dl_2$:
\begin{subequations}
\label{f}
\begin{align}
  \dd \vf_{A_1dl_1} &= \underbrace{- \int_{A_1} \int_{A_2} \rho_1(\vs_1) \rho_2(\vs_2) \pdiff{\Phi}{{\vx_{21}}} \dd A_2 \dd A_1}_{:=\vf_1} dl_2 dl_1\\
  \dd \vf_{A_2dl_2} &= \underbrace{\int_{A_1} \int_{A_2} \rho_1(\vs_1) \rho_2(\vs_2) \pdiff{\Phi}{{\vx_{21}}} \dd A_2 \dd A_1}_{:=\vf_2} dl_2 dl_1 = -\dd \vf_{A_1dl_1}
\end{align}
\end{subequations}
Here, we have defined the \textit{section-to-section} interaction forces $\vf_1$ and $\vf_2$ of dimension "force per length square". Based on the differential forces $\dd \vf_{dA_1dl_1}$ and $\dd \vf_{dA_2dl_2}$, we can define the differential moments with respect to the cross-section centroids $\vr_1$ and $\vr_2$ resulting from the interaction between the cross-section slices $A_1dl_1$ and $A_2 dl_2$:
\begin{subequations}
\label{m}
\begin{align}
  \dd \vm_{A_1dl_1|\vr_1} &= \int_{A_1} \int_{A_2}  \vs_1 \times \dd \vf_{dA_1dl_1} = \underbrace{- \int_{A_1} \int_{A_2} \rho_1(\vs_1) \rho_2(\vs_2) \vs_1 \times \pdiff{\Phi}{{\vx_{21}}} \dd A_2 \dd A_1}_{:=\vm_1} dl_2 \dd s_1\\
  \dd \vm_{A_2dl_2|\vr_2} &= \int_{A_1} \int_{A_2}  \vs_2 \times \dd \vf_{dA_2dl_2} = \underbrace{\int_{A_1} \int_{A_2} \rho_1(\vs_1) \rho_2(\vs_2) \vs_2 \times \pdiff{\Phi}{{\vx_{21}}} \dd A_2 \dd A_1}_{:=\vm_2} dl_2 dl_1
\end{align}
\end{subequations}
Here, we have defined the \textit{section-to-section} interaction moments $\vm_1$ and $\vm_2$ of dimension "moment per length square". By these definitions, the accumulated mechanical interaction between two cross-section slices $A_1 dl_1$ and $A_2 dl_2$ is given by the forces $\vf_1 dl_1 dl_2$ and $\vf_2 dl_1 dl_2$ acting at the cross-section centroids $\vr_1$ and $\vr_2$, respectively, together with the moments $\vm_1 dl_1 dl_2 $ and $\vm_2 dl_1 dl_2$.\\

In a next step, the virtual work of the interaction forces $\dd \vf_{dA_1dl_1}$ acting on point $\vx_{1}$ within cross-section $1$ and $\dd \vf_{dA_2dl_2}$ acting on point $\vx_{2}$ within cross-section $2$ shall be formulated:
\begin{align}
\label{delta_W1}
  \delta W_{int} &= \int_{l_1} \int_{l_2} \int_{A_1} \int_{A_2} \left( \delta \vx_{1}^T \dd \vf_{dA_1dl_1} + \delta \vx_{2}^T \dd \vf_{dA_2dl_2} \right).
\end{align}
Employing~\eqref{xi} and~\eqref{multi_var_base}, the virtual displacements $\delta \vx_{1}$ and $\delta \vx_{2}$ of the cross-section points $\vx_{1}$ and $\vx_{2}$ can be formulated as
\begin{align}
\label{delta_x12}
  \delta \vx_{i} &= \delta \vr_i +  \left( s_i^2  \delta \vtheta_i \times \vg_i^2 + s_i^3  \delta \vtheta_i \times \vg_i^3 \right)
  =\delta \vr_i +  \delta \vtheta_i \times \underbrace{\left( s_i^2   \vg_i^2 + s_i^3   \vg_i^3 \right)}_{\vs_i}
  =\delta \vr_i - \vS(\vs_i)\delta \vtheta_i   \quad \text{for} \quad i=1,2
\end{align}
where $\delta \vr_1$ and $\delta \vr_2$ are the variations of the two cross-section centroid positions and $\delta \vtheta_1$ and $\delta \vtheta_2$ are the spin vectors associated with the cross-section triads $1$ and $2$, respectively. Inserting~\eqref{delta_x12} in~\eqref{delta_W1} yields:
\begin{align}
\begin{split}
\label{delta_W2}
\delta W_{int} &=\int_{l_1} \int_{l_2}  \delta \vr_1^T  \int_{A_1} \int_{A_2}  \dd \vf_{dA_1dl_1}
						     + \int_{l_1} \int_{l_2} \delta \vr_2^T \int_{A_1} \int_{A_2}   \dd \vf_{dA_2dl_2}\\
						     &+ \int_{l_1} \int_{l_2} \delta \vtheta_1^T \int_{A_1} \int_{A_2} \underbrace{\vS(\vs_1) \dd \vf_{dA_1dl_1}}_{\vs_1 \times \dd \vf_{dA_1dl_1}}
						     + \int_{l_1} \int_{l_2} \delta \vtheta_2^T \int_{A_1} \int_{A_2}  \underbrace{\vS(\vs_2) \dd \vf_{dA_2dl_2}}_{\vs_2 \times \dd \vf_{dA_2dl_2}}\\
   &= \int_{l_1} \int_{l_2} \left( \delta \vr_1^\text{T} \vf_1 + \delta \vr_2^\text{T} \vf_2 + \delta \vtheta_1^\text{T} \vm_1 + \delta \vtheta_2^\text{T} \vm_2 \right) dl_1 dl_2.
\end{split}
\end{align}
As expected, the total virtual work is given by the products of the section interaction forces $\vf_i$ and moments $\vm_i$ with the associated work-conjugated virtual displacements $\delta \vr_i$ and $\delta \vtheta_i$ integrated over both beam lengths $l_1$ and $l_2$. In preparation to Section~\ref{sec:variational}, the virtual work shall be expressed as pure function of the stress resultants $\vf_2$ and $\vm_2$ acting on beam $2$. Inserting the equilibrium of forces and the equilibrium of moments w.r.t. to the cross-section centroid $\vr_1$ of beam $1$, i.e.
\begin{subequations}
\label{equilibrium}
\begin{align}
\vf_1&=-\vf_2 \label{equilibrium_1}\\
 \vm_1&=-\vm_2-(\vr_2-\vr_1) \times \vf_2 = -\vm_2-\vS(\vr_2-\vr_1) \vf_2.\label{equilibrium_2}
\end{align}
\end{subequations}
the virtual work expression~\eqref{delta_W2} can be reformulated as follows:
\begin{align}
\begin{split}
\label{delta_W3}
\delta W_{int} = \int_{l_1} \int_{l_2} \left[  \left(\delta \vr_2^\text{T} - \delta \vr_1^\text{T} \!-\!  \delta \vtheta_1^T \! \vS[\left( \vr_2 - \vr_1 \right)] \right) \vf_2 + \left( \delta \vtheta_2^\text{T} - \delta \vtheta_1^\text{T} \right) \vm_2 \right] dl_1 dl_2.
\end{split}
\end{align}
By defining the material stress-resultants in analogy to the material deformation measures as
\begin{subequations}
\label{material_stress_resultants}
\begin{align}
\vF_i&=\vLambda_1^T \vf_i \quad \text{for} \quad i=1,2 label{material_stress_resultants_1}\\
\vM_i&=\vLambda_1^T \vm_i \quad \text{for} \quad i=1,2\label{material_stress_resultants_2},
\end{align}
\end{subequations}
and inserting the identity $\vLambda_1 \vLambda_1^T$ into~\eqref{delta_W3}, also the material representation of the virtual work expression can formally be derived:
\begin{align}
\begin{split}
\label{delta_W4}
\delta W_{int} = \int_{l_1} \int_{l_2} \left[  \left(\delta \vr_2^\text{T} - \delta \vr_1^\text{T} \!-\!  \delta \vtheta_1^T \! \vS[\left( \vr_2 - \vr_1 \right)] \right) \vLambda_1 \vF_2 + \left( \delta \vtheta_2^\text{T} - \delta \vtheta_1^\text{T} \right) \vLambda_1 \vM_2 \right] dl_1 dl_2.
\end{split}
\end{align}
In the next section, the spatial and material form of the virtual work will be derived on the basis of a variational principle employing the spatial and material deformation measures $\tilde{\pi}(\vr_{21},\vpsi_{21})$ and $\tilde{\pi}(\vR_{21},\vPsi_{21})$ derived in Section~\eqref{sec:kinematics}.

\begin{center}
\begin{minipage}{0.9\textwidth}
{
\noindent \textbf{Remark:} While the equilibrium of force stress resultants~\eqref{equilibrium_1} follows directly from the definition~\eqref{f}, the equilibrium of moment stress resultants~\eqref{equilibrium_2} can alternatively be derived by integrating the moments of the differential forces $\dd \vf_{dA_1dl_1}$ and $\dd \vf_{dA_2dl_2}$ with respect to $\vr_1$ across the two interacting cross-sections:
\begin{align}
\begin{split}
  \textbf{0} &= \sum \vm_{dA_ids_i|\vr_1} = \int_{A_1} \int_{A_2}  \overbrace{\vs_1}^{\vx_1-\vr_1} \times \dd \vf_{dA_1dl_1} + \int_{A_1} \int_{A_2}  \overbrace{(\vr_2-\vr_1+\vs_2)}^{\vx_2-\vr_1} \times \dd \vf_{dA_2dl_2}  \\
  &= \int_{A_1} \int_{A_2}  \vs_1 \times \dd \vf_{dA_1dl_1} + \int_{A_1} \int_{A_2}  \vs_2 \times \dd \vf_{dA_2dl_2} + (\vr_2-\vr_1) \times \int_{A_1} \int_{A_2}  \dd \vf_{dA_2dl_2} \\
  &=\vm_1 + \vm_2 + (\vr_2-\vr_1) \times \vf_2 \quad \square
\end{split}
\end{align}
Here, from the second to the third line the definitions~\eqref{f} and~\eqref{m} have been identified.
}
\end{minipage}
\end{center}

\begin{center}
\begin{minipage}{0.9\textwidth}
{
\noindent \textbf{Remark:} Since the molecule-to-molecule interaction potential $\Phi(x)$ is only a function of the norm of $\vx_{21}$ or $\vX_{21}=\vLambda_1^T \vx_{21}$ with $x=\norm{\vx_{21}}=\norm{\vX_{21}}$, the result~\eqref{delta_W2} can equivalently be derived via variation of the total interaction potential~\eqref{potential_1} employing 
$\delta \Phi(x)=(\partial \Phi / \partial x) \delta x = (\partial \Phi / \partial \vx_{21}) \delta \vx_{21} = (\partial \Phi / \partial \vX_{21}) \delta \vX_{21}$, i.e. no objective variation $\delta_o \vx_{21}$ has to be defined for the spatial object $\vx_{21}$ (the contribution from the variation of the moving base vectors cancels out because the potential is only a function of the norm of $\vx_{21}$). It will become clear in the next section that the situation is crucially different for the deformation measures $\vr_{21}$ and $\vpsi_{21}$. There, the objective variations~\eqref{delta_o} will be required in order to formulate an equivalent representation of the principle of virtual work~\eqref{delta_W2} that is based on a variational principle and a section-to-section interaction potential $\tilde{\pi}(\vr_{21},\vpsi_{21})$ as function of the (spatial) minimal coordinates $\vr_{21}$ and $\vpsi_{21}$.
}
\end{minipage}
\end{center}


\subsection{Variational problem statement based on section-to-section interaction potential}
\label{sec:variational}

Let's consider the representation of the section-to-section interaction potential as ${\bar{\pi}}(\vR_{21},\vPsi_{21})$ as function of the material deformation measures $\vR_{21}$ and $\vPsi_{21}$ according to~\eqref{barbar_pi}. Based on~\eqref{potential_1}, the variation 
of the total interaction potential can be written as:
\begin{align}
\label{delta_Pi_material}
\delta \Pi = \int_{l_1} \int_{l_2} \left[ \frac{\partial \bar{\pi}}{\partial \vR_{21}} \delta \vR_{21} +\frac{\partial \bar{\pi}}{\partial \vPsi_{21}} \delta \vPsi_{21} \right] \dd l_2 \dd l_1.
\end{align}
Transposing the inner products in~\eqref{delta_Pi_material} and inserting the variations $\delta \vR_{21}$ and $\delta \vPsi_{21}$ from~\eqref{delta_material} yields:
\begin{align}
\begin{split}
\label{delta_Pi_material_2}
\!\!\!\!\!\delta \Pi \!&=\!\!\! \int_{l_1} \! \int_{l_2} \! \left[ \left( \delta \vr_2^T \!-\! \delta \vr_1^T \!-\!  \delta \vtheta_1^T \! \vS[\left( \vr_2 - \vr_1 \right)] \right) \vLambda_1 \! \left(\frac{\partial \bar{\pi}}{\partial \vR_{21}}\right)^{\!\!T} \!\!
+\left( \delta \vtheta_2^T \!-\! \delta \vtheta_1^T \right) \! \vLambda_1 \vT^T\!(\vPsi_{21}) \!\! \left(\frac{\partial \bar{\pi}}{\partial \vPsi_{21}}\right)^{\!\!T} \, \right] \dd l_2 \dd l_1 \!\!\!\!\! \\
								&=\!\!\! \int_{l_1} \! \int_{l_2} \! \Bigg[ \underbrace{\left( \delta \vr_2^T \!-\! \delta \vr_1^T \!-\!  \delta \vtheta_1^T \! \vS[\left( \vr_2 - \vr_1 \right)] \right) \vLambda_1}_{\delta \vR_{21}^T} \! \left(\frac{\partial \bar{\pi}}{\partial \vR_{21}}\right)^{\!\!T} \!\!
+\underbrace{\left( \delta \vtheta_2^T \!-\! \delta \vtheta_1^T \right) \! \vLambda_1}_{\delta \vTheta_{21}^T} \left(\frac{\partial_m \bar{\pi}}{\partial_m \vTheta_{21}}\right)^{\!\!T} \, \Bigg] \dd l_2 \dd l_1,\!\!\!\!\!
\end{split}
\end{align}
where from the first to the second line the definition of the multiplicative derivative according to~\eqref{multiplicative_derivative} has been identified. By considering the spatial representation of the section-to-section interaction potential ${\tilde{\pi}}(\vr_{21},\vpsi_{21})$ and employing the objective variations of the spatial deformation measures $\vr_{21}$ and $\vpsi_{21}$ according to~\eqref{delta_o}, the variation of the total interaction potential~\eqref{potential_1} can alternatively be written as 
\begin{align}
\begin{split}
\label{delta_Pi_spatial}
\!\!\!\!\!\delta \Pi \!&=\!\!\!\int_{l_1} \int_{l_2} \left[ \frac{\partial \tilde{\pi}}{\partial \vr_{21}} \delta_o \vr_{21} +\frac{\partial \tilde{\pi}}{\partial \vpsi_{21}} \delta_o \vpsi_{21} \right] \dd l_2 \dd l_1 \\ 
       &=\!\!\! \int_{l_1} \! \int_{l_2} \! \left[ \left( \delta \vr_2^T \!-\! \delta \vr_1^T \!-\!  \delta \vtheta_1^T \! \vS[\left( \vr_2 - \vr_1 \right)] \right) \! \left(\frac{\partial \tilde{\pi}}{\partial \vr_{21}}\right)^{\!\!T} \!\!
+\left( \delta \vtheta_2^T \!-\! \delta \vtheta_1^T \right) \vT^T\!(\vpsi_{21}) \!\! \left(\frac{\partial \tilde{\pi}}{\partial \vpsi_{21}}\right)^{\!\!T} \, \right] \dd l_2 \dd l_1 \!\!\!\!\! \\
								&=\!\!\! \int_{l_1} \! \int_{l_2} \! \Bigg[ \underbrace{\left( \delta \vr_2^T \!-\! \delta \vr_1^T \!-\!  \delta \vtheta_1^T \! \vS[\left( \vr_2 - \vr_1 \right)] \right)}_{\delta_o \vr_{21}^T} \! \left(\frac{\partial \tilde{\pi}}{\partial \vr_{21}}\right)^{\!\!T} \!\!
+\underbrace{\left( \delta \vtheta_2^T \!-\! \delta \vtheta_1^T \right)}_{\delta_o \vtheta_{21}^T} \! \left(\frac{\partial_m \tilde{\pi}}{\partial_m \vtheta_{21}}\right)^{\!\!T} \, \Bigg] \dd l_2 \dd l_1,\!\!\!\!\!
\end{split}
\end{align}
By comparing the spatial and material virtual work expressions~\eqref{delta_W3} and~\eqref{delta_W4} with the spatial and material variations~\eqref{delta_Pi_spatial} and~\eqref{delta_Pi_material_2}, the requirement $\delta W_{int} = \delta \Pi$ yields 
the following definition for the spatial and material stress-resultants:
\begin{subequations}
\label{stress_resultants_via_potential}
\begin{align}
\vf_2&=\left(\frac{\partial \tilde{\pi}}{\partial \vr_{21}}\right)^{\!\!T}, \quad \quad \vm_2=\left(\frac{\partial_m \tilde{\pi}}{\partial_m \vtheta_{21}}\right)^{\!\!T}=\vT^T\!(\vpsi_{21})\left(\frac{\partial \tilde{\pi}}{\partial \vpsi_{21}}\right)^{\!\!T}, \label{stress_resultants_via_potential_1}\\
\vF_2&=\left(\frac{\partial \bar{\pi}}{\partial \vR_{21}}\right)^{\!\!T}, \quad \quad \vM_2=\left(\frac{\partial_m \bar{\pi}}{\partial_m \vTheta_{21}}\right)^{\!\!T}=\vT^T\!(\vPsi_{21})\left(\frac{\partial \tilde{\pi}}{\partial \vPsi_{21}}\right)^{\!\!T}. \label{stress_resultants_via_potential_2}
\end{align}
\end{subequations}
Thus, the important result of this section is that the interaction between beams due to molecular interactions potentials and the resulting contributions to (the weak or strong form of) the mechanical balance equations can be formulated on the basis of a variational principle considering section-to-section interaction potentials ${\tilde{\pi}}(\vr_{21},\vpsi_{21})$ or ${\bar{\pi}}(\vR_{21},\vPsi_{21})$ that are a pure function of a spatial and material set of minimal coordinates. For given molecule-to-molecule interaction potentials $\Phi(x)$, the most obvious way of deriving these section-to-section interaction potentials is to perform the two cross-section integrals in~\eqref{potential_1} analytically, by setting either $x=||\vx_{21}||$ or $x=||\vX_{21}||$. Often, however, an analytical solution of these integrals (or at least of a reasonable approximation) is not possible in closed form. Alternatively, section-to-section interaction potentials as functions of the minimal coordinates $(\vr_{21},\vpsi_{21})$ or $(\vR_{21},\vPsi_{21})$ might be found via curve fitting based on values ${\tilde{\pi}}^n(\vr_{21}^n,\vpsi_{21}^n)$ or ${\bar{\pi}}^n(\vR_{21}^n,\vPsi_{21}^n)$ at discrete sampling points found experimentally or via numerical integration of the cross-section integrals.

%Noch anmerken, dass die beiden Integrale über die Balkenlänge numerisch ausgeführt werden mit Referenz auf Max's Paper

%Anmerken, dass man die Interaktionen als äußere/externe Kräfte (=Linienlasten) auf Balken 1 und 2 auffassen kann, mit den Besonderheiten:
%i) die Kräfte hängen von der Verschiebung ab
%ii) die Berechnung der Kraft an einer Stelles des einen Balken erfordert Integration über den anderen Balken

%This is an important result: 1) Simple parametrization for cases, where the integrals cannot be solved analytically: Defined parameter space that has to be sampled by means of experimental or numerical characterization. 2) Important properties (objectivity, conservation properties, existence and symmetries of solutions) follow directly from the existence of an potential associated with the mechanical problem. 3) Consistence with the geometrically exact beam theory, which has also been derived on the basis of variational principle.

\begin{center}
\begin{minipage}{0.9\textwidth}
{
\noindent \textbf{Remark:} If there is a distinct reference configuration $\vr_{21,0},\vpsi_{21,0}$ or $\vR_{21,0},\vPsi_{21,0}$, where the section-to-section interaction potential takes on a prescribed value, i.e. ${\tilde{\pi}}(\vr_{21,0},\vpsi_{21,0})={\bar{\pi}}(\vR_{21,0},\vPsi_{21,0})=0$, the deformation measures could be replaced by $\hat{\vr}_{21}= \vr_{21}-\vr_{21,0},\hat{\vpsi_{21}}=\vpsi_{21}-\vpsi_{21,0}$ or $\hat{\vR}_{21}=\vR_{21}-\vR_{21,0},\hat{\vPsi}_{21}=\vPsi_{21}-\vPsi_{21,0}$  in order to end up with a simpler expression for the section-to-section interaction potential. Of course, the additional constants would not change the variational calculus and the structure of the resulting equations as presented above.
}
\end{minipage}
\end{center}

\begin{center}
\begin{minipage}{0.9\textwidth}
{
\noindent \textbf{Remark:} Throughout this work, the cross-section triad $\vLambda_1$ has been considered as reference triad and pull-forward operator. Equivalently, material deformation measures could have been defined using $\vLambda_2$ as push-forward operator. Of course, the final virtual work expressions, i.e. the resulting weak form of the balance equations would be equivalent, with the main difference that in this case the stress-resultants on beam $1$, i.e. $\vf_1,\vm_1,\vF_1,\vM_1$ would naturally occur in the variational problem statement according to~\eqref{stress_resultants_via_potential}.
}
\end{minipage}
\end{center}



\section{Internal stored energy function as special case of SSIP laws}

There are several structural similarities in the equations derived here for the interaction of beams due to molecular interaction potentials on the basis of section-to-section interaction potentials and the equations describing the internal force and moment stress resultants in the geometrical exact beam theory on the basis of objective deformation measures related to the force and moment stress resultants via section constitutive laws, potentially derived from a section hyperelastic stored energy function. More precisely, the section-to-section interaction potentials derived here consider the interaction between two cross-sections with arbitrary relative displacement and relative rotation, while the interaction due to internal forces and moments is assumed to take place between cross-sections with centroid positions $\vr(s)$ and $\vr(s+ds)$ for the limit $ds \rightarrow 0$, where $s$ denotes the arc-length parameter along the beam centerline. These similarities shall briefly be shown by setting the centroid positions and triad orientations of the interaction cross-sections in the previously derived expressions to $\vr_1=\vr(s), \, \vpsi_1=\vpsi(s)$ and $\vr_2=\vr(s+ds), \, \vpsi_2=\vpsi(s+ds)$, and eventually considering the limit $ds \rightarrow 0$. The work-conjugated deformation measures of the internal force and moment stress resultants $\hat{\vgamma}=\vgamma-\vgamma_0, \hat{\vomega}=\vomega-\vomega_0$ in the spatial configuration and $\hat{\vGamma}=\vGamma-\vGamma_0, \hat{\vOmega}=\vOmega-\vOmega_0$ in the material configuration are defined as:
\begin{subequations}
\label{equivalence_1}
\begin{align}
\vgamma&:= \vr^{\prime}, \quad \quad \quad \,\,\, \vS(\vomega):=\vLambda^{\prime}\vLambda^T, \label{equivalence_1a}\\
\vGamma&:= \vLambda^T\vr^{\prime}, \quad \quad \vS(\vOmega):=\vLambda^T \vLambda^{\prime}, \label{equivalence_1b}
\end{align}
\end{subequations}
where $(.)^{\prime}:=d (.)/ds$ represents the derivative with respect to the arc-length coordinate $s$, and the index $(.)_0$ represents a quantity evaluated for the stress-free reference configuration. In the following, the limit $ds \rightarrow 0$ shall be considered, which equivalently means $||\vpsi_{21}||=||\vPsi_{21}|| \rightarrow 0$. In this limit, the definitions~\eqref{d_and_psi} and~\eqref{D_and_Psi} of the spatial and material relative rotation vectors yield
\begin{subequations}
\label{equivalence_2}
\begin{align}
\lim_{||\vpsi_{21}|| \rightarrow 0} (\vLambda_2-\vLambda_1)= \lim_{||\vpsi_{21}|| \rightarrow 0} (\vLambda_{21}-\vI_3)\vLambda_1= \lim_{||\vpsi_{21}|| \rightarrow 0} \vS(\vpsi_{21})\vLambda_1, \label{equivalence_2a}\\
\lim_{||\vPsi_{21}|| \rightarrow 0} (\vLambda_2-\vLambda_1)= \lim_{||\vPsi_{21}|| \rightarrow 0} \vLambda_1 (\vLambda_{\mathbbm{2}\mathbbm{1}}-\vI_3)= \lim_{||\vPsi_{21}|| \rightarrow 0} \vLambda_1 \vS(\vPsi_{21}). \label{equivalence_2b}
\end{align}
\end{subequations}
Using~\eqref{equivalence_2} and the definitions of $\vr_{21}$ and $\vR_{21}$ according to~\eqref{d_and_psi} and~\eqref{D_and_Psi}, the following relations between the proposed SIP deformation measures and the deformation measures~\eqref{equivalence_1} associated with the internal forces and moments can be established: 
\begin{subequations}
\label{equivalence_3}
\begin{align}
\vgamma& \!:=\! \vr^{\prime} \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \left[\vr(s+ds) \!-\! \vr(s) \right] \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \left[\vr_2 \!-\! \vr_1 \right] \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \vr_{21}, \label{equivalence_3a}\\
\vGamma& \!:=\! \vLambda^T \vr^{\prime} \!=\! \lim_{ds \rightarrow 0} \vLambda^T(s) \frac{1}{ds} \left[\vr(s\!+\!ds) \!-\! \vr(s) \right] \!=\! \lim_{ds \rightarrow 0}  \frac{1}{ds} \vLambda_1^T \left[\vr_2 \!-\! \vr_1 \right] \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \vR_{21}, \label{equivalence_3b}\\
\!\!\!\!\vS(\vomega)&\!:=\!\vLambda^{\prime}\vLambda^T \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \left[\vLambda(s\!+\!ds) \!-\! \vLambda(s) \right] \vLambda^T(s) \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \left[\vLambda_2 \!-\! \vLambda_1 \right] \vLambda_1^T \!=\! \lim_{ds \rightarrow 0} \vS(\frac{1}{ds} \vpsi_{21}),\!\!\!\! \label{equivalence_3c}\\
\!\!\!\!\vS(\vOmega)&\!:=\!\vLambda^T \vLambda^{\prime} \!=\! \lim_{ds \rightarrow 0} \vLambda^T(s) \frac{1}{ds} \left[\vLambda(s\!+\!ds) \!-\! \vLambda(s) \right]  \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \vLambda_1^T \left[\vLambda_2 \!-\! \vLambda_1 \right]  \!=\! \lim_{ds \rightarrow 0} \vS(\frac{1}{ds} \vPsi_{21}).\!\!\!\! \label{equivalence_3d}
\end{align}
\end{subequations}
Similar relations can be derived for the objective variations of the deformation measures occurring e.g. in the weak forms~\eqref{delta_Pi_spatial} and~\eqref{delta_Pi_material_2}, and for the definition of force and moment stress resultants via the section-to-section interaction potential in~\eqref{stress_resultants_via_potential} (note that the transformation matrix between additive and multiplicative increments becomes an identity in the considered limit $\lim_{||\vpsi_{21}|| \rightarrow 0} \vT\!(\vpsi_{21})=\vI_3$). All in all, it can be concluded that the internal force and moment stress resultants of the Simo-Reissner theory related to their work-conjugated deformation measures via section constitutive laws can be interpreted as a special case of the section-to-section interaction potentials presented here, for which only the interactions of two successive cross-sections at positions $\vr(s)$ and $\vr(s+ds)$ are considered.
%\begin{subequations}
%\label{equivalence_4}
%\begin{align}
%\delta_o \vgamma& \!:=\! \delta \vr^{\prime} \!+ \! \vS( \vr^{\prime}) \delta \vtheta_1 \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \delta_o \vr_{21}, \label{equivalence_4a}\\
%\delta \vGamma& \!:=\! \vLambda^T \left( \delta \vr^{\prime} \!+ \! \vS( \vr^{\prime}) \delta \vtheta_1 \right) \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \delta \vR_{21}, \label{equivalence_4b}\\
%\delta_o \vomega&\!:=\! \delta \vtheta^{\prime} \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \delta_o \vpsi_{21}) \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \delta_o \vtheta_{21}), \label{equivalence_4c}\\
%\delta \vOmega &\!:=\!\vLambda^T  \delta \vtheta^{\prime} \lim_{ds \rightarrow 0} \frac{1}{ds} \delta \vPsi_{21}) \!=\! \lim_{ds \rightarrow 0} \frac{1}{ds} \delta \vTheta_{21}),\label{equivalence_4d}
%\end{align}
%\end{subequations}



\section{Enforcement of translational and rotational constraints}

According to~\eqref{stress_resultants_via_potential} and~\eqref{material_stress_resultants}, the following relations have to hold between the derivatives of the spatial and material section-to-section interaction potentials:
\begin{subequations}
\label{potential_relations}
\begin{align}
\left(\frac{\partial \tilde{\pi}}{\partial \vr_{21}}\right)^{\!\!T} &= \vLambda_1 \left(\frac{\partial \bar{\pi}}{\partial \vR_{21}}\right)^{\!\!T}, \label{potential_relations_1}\\
\left(\frac{\partial \tilde{\pi}}{\partial \vpsi_{21}}\right)^{\!\!T} &= \vLambda_1 \left(\frac{\partial \bar{\pi}}{\partial \vPsi_{21}}\right)^{\!\!T}\label{potential_relations_2},
\end{align}
\end{subequations}
where for the derivation of the second equation, additionally~\eqref{multiplicative_derivative} and~\eqref{A_T1} have been used. It's straightforward to show that the relations~\eqref{potential_relations} are always fulfilled for potentials satisfying $\tilde{\pi}(\vLambda_1\vR_{21},\vLambda_1\vPsi_{21})={\bar{\pi}}(\vR_{21},\vPsi_{21})$ according to~\eqref{barbar_pi}. As a pure illustrative example, the simplest possible case of $\tilde{\pi}$ having a quadratic form shall be considered here
\begin{align}
\label{example_spatial_potential}
\!\!\! \tilde{\pi}(\vr_{21},\vpsi_{21})=\frac{1}{2}\vr_{21}^T\vc_{\vr}\vr_{21} + \frac{1}{2}\vpsi_{21}^T\vc_{\vpsi}\vpsi_{21} \,\, \rightarrow \,\,
\vf_2=\vc_{\vr}\vr_{21}, \quad \vm_2=\vT^T\!(\vpsi_{21}) \vc_{\vpsi}\vpsi_{21},\!\!\!
\end{align}
with the symmetric constants $c_{\vr}=c_{\vr}^T$ and $\vc_{\vpsi}=\vc_{\vpsi}^T$. Replacing the arguments according to $\bar{\pi}(\vR_{21},\vPsi_{21})=\tilde{\pi}(\vLambda_1 \vR_{21},\vLambda_1 \vPsi_{21})$ yields the material representation of the section-to-section interaction potential
\begin{align}
\label{example_material_potential}
\!\!\! \bar{\pi}(\vR_{21},\vPsi_{21})=\frac{1}{2}\vR_{21}^T\vC_{\vR}\vR_{21} + \frac{1}{2}\vPsi_{21}^T\vC_{\vPsi}\vPsi_{21} \,\, \rightarrow \,\, 
\vF_2=\vC_{\vR}\vR_{21}, \quad \vM_2=\vT^T\!(\vPsi_{21}) \vC_{\vPsi}\vPsi_{21}.\!\!\!
\end{align}
with $C_{\vR}=\vLambda_1^T c_{\vr} \vLambda_1$ and $C_{\vPsi}=\vLambda_1^T c_{\vpsi} \vLambda_1$. Considering e.g. a coordinate representation in the moving frame $\vg_1^i$, we get for the interaction constants:
\begin{align}
\label{constants}
\vc_{\vr}=c_{\vr}^{ij} \vg_i \otimes \vg_j^T, \,\,\,  \vc_{\vpsi}=c_{\vpsi}^{ij} \vg_i \otimes \vg_j^T, \quad \quad
\vC_{\vR}=c_{\vr}^{ij} \vE_i \otimes \vE_j^T, \,\,\,  \vC_{\vPsi}=c_{\vpsi}^{ij} \vE_i \otimes \vE_j^T.
\end{align}
It has to be emphasized, that the moments resulting from a quadratic potential according to~\eqref{example_spatial_potential} and~\eqref{example_material_potential} are not a linear function of the rotational deformation measures $\vpsi_{21}$ and $\vPsi_{21}$ in general, which directly results from the transformations $\vT\!(\vpsi_{21})$ and $\vT\!(\vPsi_{21})$ between additive and multiplicative rotation increments. In the limit of small relative rotations $\vPsi_{21} \rightarrow$ \textbf{0}, however, the transformation matrices tend to identity, i.e. $\vT\!(\vpsi_{21})\rightarrow \vI_3$ and $\vT\!(\vPsi_{21})\rightarrow \vI_3$, and the relation between moments and rotational deformation measures becomes linear.

Based on the exemplary quadratic potentials derived above, it is clear that the proposed framework can directly be used for the formulation of penalty constraints such that a prescribed relative configuration (i.e. relative orientation and distance vector) $\vR_{21,0},\vPsi_{21,0}$ between two cross-sections, or more generally between two arbitrary triads, is enforced. Replacing $R_{21}$ and $\vPsi_{21}$ in~\eqref{example_material_potential} by $\hat{\vR}_{21}=\vR_{21}-\vR_{21,0}$ and $\hat{\vPsi}_{21}=\vPsi_{21}-\vPsi_{21,0}$ directly yields such a penalty potential as well as the resulting penalty force and moment. The coupling of cross-section triads based on a penalty potential might be very beneficial for scenarios where a direct condensation of DoFs is not possible or at least involved / inefficient from a numerical point of view (e.g. coupling of two beams at non-nodal interior positions, over-constrained coupling, coupling of beam and solid finite elements at non-nodal positions).


%%
%
%\subsection{Part 2}
%
%\paragraph{Geometrical description of the mutual orientation}$\,$\\
%%
%spatial description:
%%
%\begin{align}
%  \vr_{21} := \vr_2 - \vr_1 \quad &\rightsquigarrow \quad \vr_2 = \vr_1 + \vr_{21}\\
%  \vLambda_d := \vLambda_2 \vLambda_1^\text{T} \quad &\rightsquigarrow \quad \vLambda_2 = \vLambda_d \vLambda_1 \quad \left(\text{i.\,e.~} \vg_2^j = \vLambda_d \, \vg_1^j, \, j=1,2,3 \right)
%\end{align}
%%
%material description:
%%
%\begin{align}
%  \vR_{21} &:= \vLambda_1^\text{T} \left(\vr_2 - \vr_1 \right)\\
%  \vLambda_D &:= \vLambda_1^\text{T} \vLambda_2 \quad \rightsquigarrow \quad \vLambda_2 = \vLambda_1 \vLambda_D
%\end{align}
%%
%$\rightsquigarrow$ transformation between both:
%%
%\begin{align}
%  \vR_{21} &= \vLambda_1^\text{T} \vr_{21}\\
%  \vLambda_D &= \vLambda_1^\text{T} \vLambda_d \vLambda_1 \quad \rightsquigarrow \quad \vpsi_{21} = \vLambda_1^\text{T} \vpsi_d
%\end{align}
%%
%
%\paragraph{Inter-axis potential}$\;$\\
%%
%\begin{align}
%  \vx_{21} &= \vr_2 - \vr_1 + \left( s_2^2 \vg_2^2 + s_2^3 \vg_2^3 \right) - \left( s_1^2 \vg_1^2 + s_1^3 \vg_1^3 \right)\\
%  &= \vr_{21} + \vLambda_d \left( s_2^2 \vg_1^2 + s_2^3 \vg_1^3 \right) - \left( s_1^2 \vg_1^2 + s_1^3 \vg_1^3 \right) \quad \text{with} \quad \vr_{21} = \begin{bmatrix} d^1\\ d^2\\ d^3\end{bmatrix}_{\vg_1^j}
%\end{align}
%%
%Thus, $x_{21}^j$ is a function of~$\vr_{21}$ and~$\vpsi_d$ only, and therefore~$\bar{\bar{\pi}} = \bar{\bar{\pi}}(\vr_{21}, \vpsi_d)$!
%\footnote{Note that the $s_i^j$ will be integration variables and thus result into constant values upon analytical integration over the cross-sections.}\\
%
%Now, replace~$\vx_{21}$ by~$\vLambda_1^\text{T} \vx_{21}$ (equivalent, since $\Phi=\Phi(\norm{\vx_{21}})$):
%%
%\begin{align}
%  \underbrace{\vLambda_1^\text{T} \vx_{21}}_{\vX_{21}} = \underbrace{\vLambda_1^\text{T} \vr_{21}}_{\vR_{21}} + \vLambda_D \left( s_2^2 \ve^2 + s_2^3 \ve^3\right) - \left( s_1^2 \ve^2 + s_1^3 \ve^3 \right)
%\end{align}
%%
%Thus, $X_{21}^j$ is a function of~$\vR_{21}$ and~$\vpsi_{21}$ only, and~$\pi = \pi(\vR_{21}, \vpsi_{21})$!
%
%\paragraph{Variation of the inter-axis potential}
%%
%\begin{align}
%  \pi = \pi(\vR_{21}, \vpsi_{21})
%  \quad \rightsquigarrow \quad
%  \delta \pi = \left( \pdiff{\pi}{\vR_{21}} \right)^\text{T} \delta \vR_{21} + \left( \pdiff{\pi}{{\vpsi_{21}}} \right)^\text{T} \delta \vpsi_{21}
%\end{align}
%%
%\begin{align}
%  \delta \vR_{21} = \vLambda_1^\text{T} \left( \delta \vr_2 - \delta \vr_1 + \left( \vr_2 - \vr_1 \right) \times \delta \vtheta_1 \right)
%\end{align}
%%
%\begin{align}
%  \delta \vpsi_{21} = \vT(\vpsi_{21}) \vLambda_1^\text{T} \left( \delta \vtheta_2 - \delta \vtheta_1 \right)
%\end{align}
%%
%\begin{align}
%  \delta \pi = &\left( \delta \vr_2^\text{T} - \delta \vr_1^\text{T} - \delta \vtheta_1^\text{T} \vS(\vr_2-\vr_1) \right) \vLambda_1  \overbrace{\pdiff{\pi}{\vR_{21}}}^{\vF_2}\\
%  +& \left(  \delta \vtheta_2^\text{T} - \delta \vtheta_1^\text{T} \right)\vLambda_1  \underbrace{\vT^\text{T}(\vpsi_{21}) \pdiff{\pi}{{\vpsi_{21}}}}_{\vM_2}
%\end{align}
%
%\subsection{Part 3}
%%
%\begin{align}
%  \delta \pi = \left( \delta \vr_2^\text{T} - \delta \vr_1^\text{T} \right) \vf_2 + \left( \delta \vtheta_2^\text{T} - \delta \vtheta_1^\text{T} \right) \vm_2 - \delta \vtheta_1^\text{T} \left( \left( \vr_2 - \vr_1 \right) \times \vf_2 \right)
%\end{align}
%%
%balance of forces and moments (w.\,r.\,t.~center of mass $\vr_1$):
%%
%\begin{align}
%  &\vf_1 + \vf_2 = \vnull\\
%  &\vm_2 + \vm_1 + \left( \vr_2 - \vr_1 \right) \times \vf_2 = \vnull
%\end{align}
%%
%\begin{align}
%  \rightsquigarrow \quad \vf_1 = -\vf_2, \quad \vm_1 = -\vm_2 - \left( \vr_2-\vr_1 \right) \times \vf_2
%\end{align}
%%
%\begin{align}
%  \vf_2 &= \vLambda_1 \pdiff{\pi}{\vR_{21}}, \quad \vF_2 =  \vLambda_1^\text{T} \vf_2 =  \pdiff{\pi}{\vR_{21}}\\
%  \vm_2 &= \vLambda_1 \vT^\text{T}(\vpsi_{21}) \pdiff{\pi}{{\vpsi_{21}}}, \quad \vM_2 = \vLambda_1^\text{T} \vm_2 =  \vT^\text{T}(\vpsi_{21}) \pdiff{\pi}{{\vpsi_{21}}}
%\end{align}
%%
%from (C.6) in the paper:~$\vLambda_2 \delta \vtheta_D = \delta \vtheta_2 - \delta \vtheta_1$
%%
%\begin{align}
%  \delta \pi_M =& \left( \pdiff{\pi}{{\vpsi_{21}}} \right)^\text{T} \delta \vpsi_{21}\\
%  \overset{(C.9)}{=}& \left( \pdiff{\pi}{{\vpsi_{21}}} \right)^\text{T} \vT(\vpsi_{21}) \vLambda_1^\text{T} \left(\delta \vtheta_2 - \delta \vtheta_1\right)\\
%  =& \left( \pdiff{\pi}{{\vpsi_{21}}} \right)^\text{T} \vT(\vpsi_{21}) \underbrace{\vLambda_1^\text{T} \vLambda_2}_{\vLambda_D} \delta \vtheta_D\\
%  =& \underbrace{\left( \pdiff{\pi}{{\vpsi_{21}}} \right)^\text{T} \vT(\vpsi_{21})}_{\vM_2^\text{T}} \delta_\text{L} \vtheta_D
%\end{align}
%%
%\begin{align}
%  \delta \vLambda_D &= \vLambda_D \vS(\delta \vtheta_D) =: \vS(\delta_\text{L} \vtheta_D) \vLambda_D\\
%  &\rightsquigarrow \delta_\text{L} \vtheta_D = \vLambda_D \delta \vtheta_D
%\end{align}
%
%\subsection{Part 4}
%%
%\begin{align}
%  \pi = \pi(\vR_{21}, \vpsi_{21}) \qquad \text{vs.} \qquad \bar{\bar{\pi}} = \bar{\bar{\pi}}(\vr_{21}, \vpsi_d)
%\end{align}
%%
%Note: not so happy with this notation since the tilde indicates a length-specific quantity; I think, we need another symbol for material vs. spatial function
%%
%\begin{align}
%  \delta \pi_M &= \delta \vpsi_{21}^\text{T} \pdiff{\pi}{{\vpsi_{21}}}
%  = \underbrace{\delta \vtheta_D^\text{T}}_{\left(\vLambda_1^\text{T} \left(  \delta \vtheta_2 - \delta \vtheta_1\right) \right)^\text{T} }  \underbrace{\vT^\text{T}(\vpsi_{21}) \pdiff{\pi}{{\vpsi_{21}}}}_{\vM_2 = \pdiff{\pi}{{\vtheta_D}} }
%\end{align}
%
%\begin{align}
%  \delta \bar{\bar{\pi}}_M &= \delta_\text{o} \vpsi_d^\text{T} \pdiff{\bar{\bar{\pi}}}{{\vpsi_d}}
%  = \underbrace{\delta \vtheta_d^\text{T}}_{ \left(  \delta \vtheta_2 - \delta \vtheta_1\right)^\text{T} }  \underbrace{\vT^\text{T}(\vpsi_d) \pdiff{\bar{\bar{\pi}}}{{\vpsi_d}}}_{\vm_2 = \pdiff{\bar{\bar{\pi}}}{{\vtheta_d}} }
%\end{align}
%%
%with~$\vpsi_d = \vLambda_1 \vpsi_{21}$:
%%
%\begin{align}
%  \delta \vpsi_d = \underbrace{\vLambda_1 \delta \vpsi_{21}}_{\delta_\text{o} \vpsi_d} + \delta \vtheta_1 \times \vpsi_d
%\end{align}
%%
%\begin{align}
%  \delta_\text{o} \vpsi_d &= \vLambda_1 \delta \vpsi_{21}\\
%  \delta_\text{o} \vtheta_d &= \vLambda_1 \delta \vtheta_D
%\end{align}





